LVC: A Lightweight Compression Framework for Enhancing VLMs in Long Video Understanding

Long video understanding is a complex task that requires both spatial detail and temporal awareness. While Vision-Language Models (VLMs) obtain frame-level understanding capabilities through multi-frame input, they suffer from information loss due to the sparse sampling strategy. In contrast, Video Large Language Models (Video-LLMs) capture temporal relationships within visual features but are limited by the scarcity of high-quality video-text datasets. To transfer long video understanding capabilities to VLMs with minimal data and computational cost, we propose Lightweight Video Compression (LVC), a novel method featuring the Query-Attention Video Compression mechanism, which effectively tackles the sparse sampling problem in VLMs. By training only the alignment layer with 10k short video-text pairs, LVC significantly enhances the temporal reasoning abilities of VLMs. Extensive experiments show that LVC provides consistent performance improvements across various models, including the InternVL2 series and Phi-3.5-Vision. Notably, the InternVL2-40B-LVC achieves scores of 68.2 and 65.9 on the long video understanding benchmarks MLVU and Video-MME, respectively, with relative improvements of 14.6% and 7.7%. The enhanced models and code will be publicly available soon.

==> sec/2_formatting.tex <==
\section{Formatting your paper}
\label{sec:formatting}

All text must be in a two-column format.
The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
Columns are to be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
The second and following pages should begin 1 inch (2.54 cm) from the top edge.
On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
high.
%
Page numbers should be in the footer, centered and $\frac{3}{4}$ inches from the bottom of the page.
The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
The \LaTeX\ template takes care of this when used properly.



%-------------------------------------------------------------------------
\subsection{Type style and fonts}

Wherever Times is specified, Times Roman may also be used.
If neither is available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE.
Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
Leave two blank lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type.
This information is to be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT.
Type main text in 10-point Times, single-spaced.
Do NOT use double-spacing.
All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
Make sure your text is fully justified---that is, flush left and flush right.
Please do not place any additional blank lines between paragraphs.

Figure and table captions should be 9-point Roman type as in \cref{fig:onecol,fig:short}.
Short captions should be centred.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

FIRST-ORDER HEADINGS.
(For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before, and one blank line after.

SECOND-ORDER HEADINGS.
(For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before, and one after.
If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use footnotes\footnote{This is what a footnote looks like.
It often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{Cross-references}

For the benefit of author(s) and readers, please use the
{\small\begin{verbatim}
  \cref{...}
\end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross-reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, please see \cref{fig:onecol} and \cref{tab:example}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
  You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
\end{quotation}
If you do not wish to abbreviate the label, for example at the beginning of the sentence, you can use the
{\small\begin{verbatim}
  \Cref{...}
\end{verbatim}}
command. Here is an example:
\begin{quotation}
  \Cref{fig:onecol} is also quite important.
\end{quotation}

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
When referenced in the text, enclose the citation number in square brackets, for
example~\cite{Authors14}.
Where appropriate, include page numbers and the name(s) of editors of referenced books.
When you cite multiple papers at once, please make sure that you cite them in numerical order like this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
If you use the template as advised, this will be taken care of automatically.

\begin{table}
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
  \caption{Results.   Ours is better.}
  \label{tab:example}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
Instead use
{\small\begin{verbatim}
  \centering
\end{verbatim}}
at the beginning of your figure.
Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it's almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
Hence avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

==> sec/3_finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.

==> sec/3_method.tex <==
\section{Methods}

\subsection{Model Architecture}
\begin{figure}[h]
  \centering
   \includegraphics[width=\linewidth]{images/1.png}

   \caption{(a)VLMs (b)Video-LLMs (c)The overall architecture of LVC}
\end{figure}

LVC is designed to extend VLMs for long video understanding with minimal training cost. 
As shown in Figure 1(c), the overall architecture integrates multi-frame temporal information through a Visual Encoder, a parameter-free compression module, an MLP-based alignment layer, and the LLM backbone. 

VLMs in Figure 1(a) typically understand videos through sparse frame sampling combined with multi-image reasoning, which leads to insufficient information for long video understanding. 
By contrast, Video-LLMs in Figure 1(b) densely sample frames and employ visual compression modules. However, these methods require joint training of the compression module, alignment layers, and LLM itself, demanding large amounts of data and high computational costs. 
Despite their complexity, Video-LLMs exhibit no significant performance advantage over high-quality VLMs like Qwen2-VL.

To retain the efficiency of VLMs while overcoming their limitations, we propose a lightweight adaptation strategy LVC, extending VLMs for long video understanding. 
Specifically, LVC introduces denser frame sampling to capture fine-grained temporal information and then compresses them into "pseudo-images" \red{TODO: explain pseudo-images} through the parameter-free compression module. 

The only trainable component is the MLP-based alignment layer, which projects compressed features into the text space of the LLM backbone. 
This design allows the pre-trained VLM to rapidly adapt to long video inputs without finetuning the VLM, achieving both parameter efficiency and temporal modeling capability. \red{TODO: revise}

In terms of computational complexity, our method increases only the Visual Encoder’s computation, while keeping LLM-side processing unchanged, offering a novel solution for long-video understanding.

\subsection{Providing more Frames for Better Video Understanding}
General video understanding tasks can be formulated as: given a video $v$ and a textual query $q$, the goal is to predict a textual answer $a$.
VLMs process the video into $N$ sampled frames $f_1, f_2,...,f_N$.
These sampled frames are processed through a Vision Transformer, such as CLIP-ViT, to obtain sampled frame features $F_1, F_2,...,F_N, F_i \in \mathbb{R}^{t \times d}$. Here, $t$ represents the number of tokens describing an image frame, and $d$ denotes the feature dimension of each token.

The sampled frame features $F_{i, i=1,...,N}$ are sequentially concatenated along the token dimension and aligned to the LLM's text space using an alignment layer. 
They are then concatenated with the query embedding $Q \in \mathbb{R}^{l \times d'} $ and fed into the LLM for autoregressive decoding to generate the answer.


\begin{equation}
  V = \text{Align}([F_1; F_2; \dots; F_N]) \in \mathbb{R}^{(N t) \times d'}
\end{equation}

\begin{equation}
    P(Y | V, Q) = \Pi_{j=1}^L P_{LLM}(Y_j | V, Q, Y_{i<j})
\end{equation}

Here, $d'$ represents the feature dimension in the LLM's text space, $V$ represents the input visual features, and $Y_{i<j}$ represents the text embeddings generated from previous outputs.

Video-LLMs densely sample $M$ frames and apply feature compression on the sampled frame features. The input feature token length must account for the window size limitation of the LLM backbone; therefore, in typical VLMs, $N$ is generally set to 8 or 16.

LVC compresses densely sampled frames into a form that matches the shape of the visual feature input $V$ in VLMs, thus referring to them as pseudo-image frames.
This serves as a method to enhance the information content of VLM inputs. 
While similar in principle to the compression modules in Video-LLMs, LVC does not rely on data-driven pre-training and fine-tuning.

\subsection{Infusing Queries into Video Compressing}
Densely sampled frames often contain redundant information, and directly concatenating real frame features in sequence would far exceed the LLM input limitation.
To address this, we propose a Query-Attention Video Compressing mechanism, which leverages the text modality to retain essential information needed for video understanding.

Specifically, the densely sampled frames are processed through a Vision Transformer and alignment layer to obtain the visual features $V$. Based on the compression ratio, a window length $w$ is set, and $V$ is sliced as:

\begin{equation}
    V = [V_1,V_2,...,V_w], V_i \in R^{\frac{Mt}{w} \times d'}, i=1,...,w
\end{equation}

$V_i$ represents the local video features, where the video is divided into windows to ensure that the temporal information of the video is preserved.
The textual query $q$ with length $l$ is passed through a Text Embedding layer to obtain the query features $Q \in R^{l \times d'}$, and then the token dimension is averaged to derive the sentence-level query feature:

\begin{equation}
    \overline{Q} = \frac{1}{l} \sum_{i=1}^l Q_i, Q_i \in R^{d'}
\end{equation}

The query feature $\overline{Q}$ is integrated into $V$ by generating weights, which are then used to modulate the visual features: \red{TODO: add multi-head and softmax}

\begin{equation}
    W_i = V_i \cdot \overline{Q} \in R^{\frac{Mt}{w}}
\end{equation}

\begin{equation}
    V' = \sum_{i=1}^w W_i \cdot V_i \in R^{\frac{Mt}{w} \times d'}
\end{equation}

Here, $M' = M/w$ represents the number of frames after compression. When $M$ is divisible by $w$, the compressed visual features $V'$ align with the shape of $M'$ image frames. Therefore, we refer to these as pseudo-image frames, which can be quickly learned by the alignment layer of the VLM with a small amount of data.

Additionally, we observe that the multi-head mechanism introduces more multi-modal weight information in the compression process. The pseudo-code for our complete compression mechanism is as follows: \red{TODO: code}

\label{sec:methods}
